A Tight 4/3 Approximation for Capacitated Vehicle Routing in Trees

Given a set of clients with demands, the Capacitated Vehicle Routing problem is to find a set of tours that collectively cover all client demand, such that the capacity of each vehicle is not exceeded and such that the sum of the tour lengths is minimized. In this paper, we provide a 4/3-approximation algorithm for Capacitated Vehicle Routing on trees, improving over the previous best-known approximation ratio of $(\sqrt{41}-1)/4$ by Asano et al., while using the same lower bound. Asano et al. show that there exist instances whose optimal cost is 4/3 times this lower bound. Notably, our 4/3 approximation ratio is therefore tight for this lower bound, achieving the best-possible performance.

==> tex/conclusion.tex <==
\section{Conclusion}

==> tex/draft.tex <==

\section{Intro}


Givem a graph $G = (V,E)$, specified depot vertex $r$, demand function $d: V
\rightarrow \mathbb{R}^{\geq 0}$ and $Q>0$, the {\sc Vehicle Routing} problem
is to find a set of tours of minimum total length such that the tours collectively
\emph{cover} all demand at every vertex and such that no tour covers more than $Q$
demand.



\begin{itemize}
\item previous work on vehicle routing (and capacitated multicast?)
\item emphasize that this shows tightness with lower bound
\item describe Asano's technique and how this generalizes
\end{itemize}


\section{Preliminaries}




approximations

OPT

parent, child of vertices and edges

When the input graph $G$ is a tree it is assumed to be rooted at the depot $r$.

For rooted tree $T=(V,E)$, and $v\in V$ let $T_v$ denote the subtree rooted
at $v$ and $d(T_v)$ be the total demand from vertices in $T_v$.  An edge labeled $
(u,v)$ indicates that $u$ is the parent of $v$.  If $v$ has parent
vertex $u$, we call $B_{uv} = T_v \cup \{(u,v)\}$ the
$v$-\emph{branch} at $u$, and edge $(u,v)$ the \emph{stem} of the branch.

\subsection{Lower Bound}
Since all demand must be covered and each tour can cover at most $Q$ demand, each
edge $e = (u,v)$ must be traversed by enough tours to cover $d(T_v)$ demand.  
We call this value the \emph{traffic} on the edge $e$, denoted $f(e)$.
Namely,
$f(e) = \lceil\frac{d(T_v)}{Q}\rceil$ tours.   Each such tour
traverses the edge exactly twice
(once in each direction).  We say that the lower bound $LB(e)$ of the contribution
of edge $e = (u,v)$ to the total solution cost is therefore,  $$LB(e) = 2\cdot l(e)\cdot
f(e) = 2\cdot l(e)\lceil
\frac{d(T_v)}{Q}\rceil$$ and that the lower bound $LB$ on $OPT$ is $$LB
= \sum_{e\in E}LB(e)$$.


For convenience, we scale down all demand values by a factor of $Q$ and set $Q=1$.
We also assume that the vertices with positive demand are exactly the leaves:  If
some internal vertex $v$ has positive demand $d(v)$ we can add a vertex $v'$ with
demand $d(v') = d(v)$ and edge $(v,v')$ of length zero and set $d(v)$ to zero. Alternatively,
if some leaf $v$ has zero demand, no tour in an optimal solution will visit $v$ so
$v$ and the edge to $v$'s parent can be deleted from the graph.


A very high level description of the algorithm is as follows: iteratively identify
(and remove) groups of tours
in which the ratio of the cost of the tours to the reduction in cost to the lower bound,
$LB$, is at most $4/3$.  We call such a set of tours a $4/3$-\emph{approximate tour
group}.

\begin{lemma}\label{lem:tours}
If, after traversing all tours in some set of $4/3$-approximate tour groups,
no
demand remains, then
the resulting set of tours is a $4/3$-approximation for {\sc Capacitated Vehicle Routing}.
\end{lemma}


Given this, we make one more simplifying assumption that each leaf $v$ has demand
$d(v) < 1$. Assume to the contrary that for some leaf $v$, $d(v) \geq 1$.  A tour
that goes directly from $s$ to $v$ and back and covers one unit of demand at $v$ is
in fact a 1-approximate tour (and thus also a $4/3$-approximate tour).  If ever such
a leaf exists, we can greedily take such tours until no more such leaves exist.


\subsection{Safe Operations}
We say that an operation that modifies the graph is \emph{safe} if it does not decrease
$OPT$
and does not change the cost of the lower bound $LB$.  Note that a $4/3$-approximate
tour in the modified graph is therefore also a $4/3$-approximate tour in the unmodified
graph.

The algorithm proceeds iteratively.  In each iteration, the algorithm performs a series
of \emph{safe} operations and takes a sequence of $4/3$-approximate tours.

We now define the operations.  Note that many of these operations also appear in 
\cite{asano} with different vocabulary \comment{map these onto Asano's?}.

\begin{itemize}
\item {\bf Condense}:  If edge $e = (u,v)$ has traffic $f(e) = 1$ and $v$ is not a
leaf, add a vertex $v'$ and replace $e$ and $T_v$ with an edge $e'= (u,v')$ with $l
(e') = l(e) + \sum_{e''\in T_v}l(e'')$ and set $d(v') = d(T_v)$ (see Figure~\ref{fig:condense}).
 The traffic of all edges in $T_v$ must have been one, and their lengths are summed
 with $l(e)$ to give $l(e')$, so the entire contribution to $LB$ is constant. Note
 that this modification may increase $OPT$ because it is equivalent to requiring a
 tour that visits any vertex in $T_v$ to traverse the entire subtree.
 \item {\bf Unzip}: If edge $e = (u,v)$ has traffic equal to the sum of the traffic
 on child edges $(v,w_1),(v,w_2),...,(v,w_k)$, then delete $v$ and add edges $(u,w_1),
 (u,w_2),...,(u,w_k)$ with lengths $l((u,w_i))=l(e)+l(v,w_i)$ for all $i \in \{1,2,...,k\}$
 (see Figure~
\ref{fig:unzip}).  The former contribution $LB(e)$ of $e$ to the lower bound is now
distributed across the newly added edges, so $LB$ is preserved.  Note that $v$ is
an internal vertex and has been assumed to have zero demand.
 \item {\bf Group}:  If vertex $u$ has children $v_1,v_2,...,v_k$, add vertex $u'$,
 edge $(u,u')$ of length zero, and for any $i\leq k$, replace $(u,v_j)$ with $(u',v_j)$
 for all $j \in \{1,2,...,i\}$ (see Figure~\ref{fig:group}).
\item {\bf Unite}: If vertex $u$ has leaf children $v_1$ and $v_2$ such that $d(v_1)
+ d(v_2) \leq 1$ \comment{< or $\leq$?}, delete $v_1$ and $v_2$ and add vertex $v_0$
with demand $d(v_1)+d(v_2)$
and edge $(u,v_0)$ with length $l((u,v_1))+l((u,v_2))$ (see Figure~\ref{fig:unite}).
 Note that this operation is equivalent to a \emph{group} followed by a \emph{condense}.
\item {\bf Slide}: If edge $e_0 = (u,v)$ has child edges $ e_1 = (v,w_1)$ and $e_2
= (v,w_2)$ such that traffic $f(e_0) = f(e_1)$, then delete vertex $v_1$ and add edge
$(u,w_1)$ of length $l(e_0)+l(e_1)$ and edge $(w_1,w_2)$ of length $l(e_2)$ (see Figure~
\ref{fig:slide}).
\end{itemize}

Since these operations are always \emph{safe}, the algorithm performs them whenever
available, with the caveat that a \emph{group} operation is not performed if it is
immediately \emph{unzip}-able. \comment{need to show that this terminates? need to
discuss maintaining simplification assumptions?}


\section{Algorithm}
We say that a problem instance is \emph{simplified} if no more safe operations are
available (except, as mentioned above, unzip-able \emph{group} operations), no internal
vertices have demand, and for every leaf $v$, $0 < d(v) <1$.

Recall that a \emph{branch} consists of a subtree along with its parent edge (\emph{stem}).
 If the branch has traffic $p$, we call it a $p$-\emph{branch}.



A 2-branch with stem $e_0 = (u,v)$ such that $v$ has exactly three children $w_1,w_2,w_3$,
all of which are leafs and such that $1.5 < d(w_1)+d(w_2)+d(w_3) < 2$ is called a
$2$-\emph{chain} (see Figure~\ref{fig:2_chain}). %\comment{< 2 or \leq 2}


\begin{lemma}\label{lem:2_chain}
In a simplified problem instance, all 2-branches are 2-chains.
\end{lemma}

\begin{proof}
Consider any 2-branch in a simplified problem instance.  Clearly no edge in the branch
can have traffic greater than
 two.  If more than one child edge of the stem had traffic two, then the traffic of
 the stem itself must be greater than two.  If the stem had exactly one child edge
 with traffic two, then a slide operation would have been possible. Therefore every
 child edge of the stem has traffic one. Each of these edges must be leaf edges or
 else they could be condensed.  If there were exactly two such
 edges, then
 the stem could be unzipped.  Since no two of these edges can be united, then the
 demand of every pair sums to more than one, so there are exactly three such edges
 and their demand sums to more than 1.5.
\end{proof}

We now generalize the notion of a 2-chain.  For $p \geq 3$, a $p$-\emph{chain} is a
$p$-branch
with stem $e_0 = (u,v)$ such that $v$ has exactly three children $w_1,w_2,w_3$, in
which $w_2$ and $w_3$ are leaves with $1<d(w_2)+d(w_3)<1.5$ and $(v,w_1)$ is the stem
of a $(p-1)$-chain (see Figure~\ref{fig:p_chain}).%\comment{< 1.5 or \leq 1.5}

\comment{need no slide operations to be available.  not sufficient definition for
p-chain}

For convenience, we define a labeling scheme for $p$-chains.  Each vertex $v_i^j$
is doubly
indexed by level $i$ and rank (child-order) $j$.  We use $e_i^j$ to denote the parent
edge of $v_i^j$, $\forall i,j$. A $2$-chain with parent $u$
has stem $e_2^0=(u,v_2^0)$ leaves $v_1^0$, $v_1^1$, and $v_1^2$ such that $l(e_1^0) \geq
l
(e_1^1) \geq l
(e_1^2)$.  For $p>2$, a $p$-chain with parent $u$
has stem $e_p^0=(u,v_p^0)$, and children $v_{p-1}^0$, $v_{p-1}^1$, and $v_{p-1}^2$, such
that $e_{p-1}^0$ is the stem of a $(p-1)$-chain, and $v_{p-1}^1$ and $v_{p-1}^2$ are
leaves with $l(e_{p-1}^1) \geq l(e_{p-1}^2$ (See Figure~\ref{fig:chain_label}).


Furthermore, we classify some $p$-chains as \emph{long}.  All $2$-chains are long
and for $p \geq 3$ a \emph{long} $p$-\emph{chain} is a
$p$-chain in which $l(e_{p-1}^2) < 3l(e_p^0)$ and $e_{p-1}^0$
is the stem of a \emph{long} $(p-1)$-chain (see Figure~\ref{fig:long_p_chain}).


\comment{need to define some concept of removing branches/demand}

Long $p$-chains are particularly convenient because they can be \emph{removed}
individually at the root, and \emph{removed} as sibling pairs at internal tree nodes.


The labeling on $p$-chains gives a natural bottom-up ordering on the leaves: $v_1^0,v_1^1,v_1^2,v_2^1,v_2^2,...,v_
{p-1}^1,v_{p-1}^2$, where the order is determined first by level and then by rank.
For a long $p$-chain, we define a \emph{cascade} to be the sequence of $p$
tours in which each tour considers the leaves in this bottom-up order and:
\begin{itemize}
\item visits and covers all demand from the first leaf with remaining demand
\item while the vehicle has spare capacity and there is unmet demand in the branch,
determines the lowest level $i$ with leaves
with unmet demand and covers as much demand as possible from $v_i^2$.
\item returns to the depot
\end{itemize}

Let the resulting tours be $t_1,...,t_p$.  Tour $t_1$ first covers all demand from
$v_1^0$ and then covers $1-d(v_1^0)$ demand from $v_1^2$.  Since the unite operation
is unavailable,\comment{need to specify this in the definition} $d(v_1^0)+d(v_1^2)
> 1$ so the vehicle is full.  The second tour $t_2$ covers all demand from $v_1^1$,
covers all remaining demand at $v_1^2$ (since $d(v_1^0)+d(v_1^1)+d(v_1^2)
< 2$) and covers some demand at $v_2^2$.  Since the slide operation is unavailable,
$d(v_1^0)+d(v_1^1)+d(v_1^2) +d(v_2^2)
> 3$, so the vehicle is full.  Note that $t_1$ and $t_2$ have both been at full capacity, and after these two tours no demand
remains at level $1$.  This pattern continues. Tour $t_i$ for $3 \leq i < p$ covers
all demand at $v_{i-1}^1$, all remaining demand at $v_{i-1}^2$, and some demand at
$v_i^2$.  Again, since slide operation is unavailable and all previous vehicles have
been full, this vehicle must also be full.  After $t_i$, no demand remains below level
$i$.  Since all vehicles have been full, there is less than one unit of demand remaining
for $t_p$ (and no demand remains below level $p-1$), so $t_p$ covers all demand from
$v_{p-1}^1$ and all remaining demand from $v_{p-1}^2$. (See Figure~\ref{fig:cascade}).

This cascading pattern results in $i$ tours traversing $e_i^0$,
one tour traversing $e_i^1$ (and $e_1^0$), two tours traversing $e_i^2$ for all
$i$, and $p$ tours traversing all edges in the path from the depot $r$ to $v_p^0$.
Note in particular that these values match the lower bounds given by the edge
traffic, for $e_i^0$ and $e_i^1$.  The excess cost, therefore, comes from doubling
the traffic lower bound on the $e_i^2$ edges as well as 



in
pairs.  In particular, if vertex $v$ has two distinct child branches $B_1$ and $B_2$
such that $B_1$ is a long $p_1$-chain and $B_2$ is a long $p_2$-chain, 





The algorithm proceeds in a series of iterations, one for each $i$ in $\{1,2,...,m\}$,
where $m = \lceil D(T)\rceil$ is the total demand of the instance.  Each iteration
performs a set of safe operations and identifies a collection of $4/3$-approximate
tours until the result of Lemma~\ref{lem:iteration} holds.


\begin{lemma}\label{lem:iteration}
For all $i$ in $\{3,4,...,m\}$, iteration $i$ runs in polynomial time, and at the end of iteration $i$, all remaining $p$-branches are long $p$-chains for
all $p \in \{2,3,...,i\}$.
\end{lemma}
\begin{proof}
See Section~\ref{sec:iteration}.
\end{proof}

Once all iterations have completed, the algorithm solves the remaining instance, using
the result from Lemma~\ref{lem:root}

\begin{lemma}\label{lem:root}
There is a polynomial-time $4/3$-approximation algorithm for instances of {\sc Vehicle Routing} on
trees in which every child branch of the root is either a long $p$-chain or a 1-branch.
\end{lemma}
\begin{proof}
See Section~\ref{sec:root}.
\end{proof}

Putting these steps together, gives our overall 4/3-approximation result described
in Theorem~\ref{thm:main}.


\begin{theorem}\label{thm:main} There is a polynomial-time 4/3 approximation for 
{\sc Vehicle
Routing} in trees.
\end{theorem}
\begin{proof}
Let $m$ denote the total amount of demand in the graph. The maximum traffic on any edge is therefore $m$.  By Lemma~\ref{lem:iteration} then,
after iteration $m$, every branch off the root must be a long $p$-chain or
a 1-branch.  By Lemma~\ref{lem:root} there is a $4/3$ approximation for these branches.
Combining this approximation with the collection of tours identified during the iterations
results in an overall $4/3$ approximation, by \ref{lem:tours}.  As each iteration runs in polynomial time, the overall runtime is polynomial.
\end{proof}

All that remains is to describe the iteration subroutine and to prove Lemmas~\ref{lem:iteration}~and~
\ref{lem:root}, as we do in the following two sections. 

\section{Description of Iteration $i$}\label{sec:iteration}


Consider iteration for $i >2$.  By induction we assume that Lemma~\ref{lem:iteration}
holds for $i-1$, therefore all $j$-branches for $j\in \{2,...,i-1\}$ are long $j$-chains
(the base case for the induction is given by Lemma~\ref{lem:2_chain} since all 2-chains
are long).  If every $i$-branch is a long $i$-chain, then the current iteration  is
terminated.  Otherwise there exists some $i$-branch $B$ such that all child branches
of
the stem are either long $j$-chains for $2\leq j< i$ or $1$-branches.

We say that a $j$-branch that is not a long $j$-chain is \emph{untreated}.

Simplify the instance.

If there is some untreated $j$-branch $j$ in $\{3,...,i\}$, find an untreated $j$-branch $B$, such that none of the child branches are untreated.  That is, every child branch of $B$ is either a long $p$-chain for some $p<j$, or is a 1-branch. 

If $B$ has more than one long $p$-chain child branch, remove them in pairs, using \sc{remove\_p\-chain\_pair}, until at most one long $p$-chain child branch remains.

If $B$ has more than three 1-branches, remove triples using \sc{remove\_1\-branch\_triple} until at most two 1-branches remain as child branches.



\subsection{Removing Long $p$-Chain Pairs}

\begin{lemma}
If some vertex $v$ has child branches $B_1$ and $B_2$ such that $B_1$ is a long $p_1$-chain and $B_2$ is a long $p_2$-chain, then $B_1$ and $B_2$ can be removed.
\end{lemma}
\begin{proof}


The labeling on $p$-chains gives a natural bottom-up ordering on the leaves: $v_1^0,v_1^1,v_1^2,v_2^1,v_2^2,...,v_
{p-1}^1,v_{p-1}^2$, where the order is determined first by level and then by rank.
For a long $p$-chain, we define a \emph{cascade} to be the sequence of $p$
tours in which each tour considers the leaves in this bottom-up order and:
\begin{itemize}
\item visits and covers all demand from the first leaf with remaining demand
\item while the vehicle has spare capacity and there is unmet demand in the branch,
determines the lowest level $i$ with leaves
with unmet demand and covers as much demand as possible from $v_i^2$.
\item returns to the depot
\end{itemize}

Let the resulting tours be $t_1,...,t_p$.  Tour $t_1$ first covers all demand from
$v_1^0$ and then covers $1-d(v_1^0)$ demand from $v_1^2$.  Since the unite operation
is unavailable,\comment{need to specify this in the definition} $d(v_1^0)+d(v_1^2)
> 1$, so the vehicle is full.  The second tour $t_2$ covers all demand from $v_1^1$,
covers all remaining demand at $v_1^2$ (since $d(v_1^0)+d(v_1^1)+d(v_1^2)
< 2$) and covers some demand at $v_2^2$.  Since the slide operation is unavailable,
$d(v_1^0)+d(v_1^1)+d(v_1^2) +d(v_2^2)
> 3$, so the vehicle is full.  Note that $t_1$ and $t_2$ have both been at full capacity, and after these two tours no demand
remains at level $1$.  This pattern continues. Tour $t_i$ for $3 \leq i < p$ covers
all demand at $v_{i-1}^1$, all remaining demand at $v_{i-1}^2$, and some demand at
$v_i^2$.  Again, since slide operation is unavailable and all previous vehicles have
been full, this vehicle must also be full.  After $t_i$, no demand remains below level
$i$.  Since all vehicles have been full, there is less than one unit of demand remaining
for $t_p$ (and no demand remains below level $p-1$), so $t_p$ covers all demand from
$v_{p-1}^1$ and all remaining demand from $v_{p-1}^2$. (See Figure~\ref{fig:cascade}).

This cascading pattern results in $i$ tours traversing $e_i^0$,
one tour traversing $e_i^1$ (and $e_1^0$), two tours traversing $e_i^2$ for all
$i$, and $p$ tours traversing all edges in the path from the depot $r$ to $v_p^0$.
Note in particular that these values match the lower bounds given by the edge
traffic, for $e_i^0$ and $e_i^1$.  The excess cost, therefore, comes from doubling
the traffic lower bound on the $e_i^2$ edges as well as 


The total cost of the cascade is therefore:

$$ p\cdot l(r,v_p^0) + l(e_1^0) + \sum_{i=1}^p l(e_i^1) + \sum_{i=1}^p 2l(e_i^2) + + \sum_{i=2}^p i\cdot l(e_i^0)$$

The reduction to the cost of $LB$ is

$$ p\cdot l(r,v_p^0) + l(e_1^0) + \sum_{i=1}^p l(e_i^1) + \sum_{i=1}^p 2l(e_i^2) + + \sum_{i=2}^p i\cdot l(e_i^0)$$





\end{proof}

{\sc remove\_p\-chain\_pair}



\begin{itemize}
\item while there is a $j$-branch, $j\geq i$ (maybe not? don't want to cause any new
$j$-branches of small $j$) that is not a $j$-chain,
\item B = minimal such $j$-branch
\item By induction, all sub-branches are $p$-chains for $p < i$ or 1-branches
\item Remove $p$-chains in pairs, using \sc{remove\_p\-chain\_pair}
\item Remove excess 1-branches using \sc{remove\_1\-branches}
\end{itemize}

\section{Proof of Lemma~\ref{lem:root}}\label{sec:root}


\section{Conclusion}







